One-Sided Expert-Parallel All-to-All for Mixture-of-Experts Inference over NVLink

Expert parallelism (EP) shards the experts of a Mixture-of-Experts (MoE) layer across GPUs, so every MoE layer requires two all-to-all communications, namely dispatch and combine. Compared with training, inference processes relatively few tokens per GPU at a time, and at small batch sizes fixed costs that do not grow with the number of tokens, rather than data movement, dominate the latency. We present NVLinkOneSided, a one-sided EP all-to-all for GPUs within a single NVLink domain. Each source rank pushes its tokens, without first exchanging metadata, into rank-major buffers on the target GPUs, and the grouped GEMMs read them in place instead of from a per-expert copy. We provide two protocols for the synchronization that the communication requires, namely Fence and Sentinel, for high-throughput and low-latency scenarios respectively. On Blackwell GPUs, NVLinkOneSided completes dispatch and combine 1.2-3.0$\times$ faster than DeepEP, with the largest speedups at small batch sizes. The resulting MoE layer is up to 2.4$\times$ faster than DeepEP with DeepGEMM. It even outperforms the fused DeepGEMM MegaMoE at up to 128 tokens per GPU, making it still competitive for decoding. We expose NVLinkOneSided through a modular interface, so that it is agnostic to the activation quantization format, decoupled from the MoE compute backend and easy to integrate into inference frameworks.

==> generated/table_b300_kimik3.tex <==
    1 & \prelim{8.6} & \prelim{8.6} & \prelim{17.2} & \prelim{12.7} & \prelim{11.3} & \prelim{24.0} & \prelim{23.2} & \prelim{26.2} & \prelim{49.3} \\
    2 & \prelim{8.9} & \prelim{8.7} & \prelim{17.6} & \prelim{13.0} & \prelim{11.2} & \prelim{24.2} & \prelim{23.8} & \prelim{29.0} & \prelim{52.8} \\
    4 & \prelim{8.7} & \prelim{11.1} & \prelim{19.7} & \prelim{12.4} & \prelim{11.5} & \prelim{23.9} & \prelim{25.1} & \prelim{29.9} & \prelim{55.0} \\
    8 & \prelim{9.0} & \prelim{11.5} & \prelim{20.5} & \prelim{13.2} & \prelim{11.3} & \prelim{24.4} & \prelim{24.4} & \prelim{30.8} & \prelim{55.2} \\
    16 & \prelim{9.2} & \prelim{11.7} & \prelim{20.9} & \prelim{13.1} & \prelim{14.0} & \prelim{27.2} & \prelim{25.0} & \prelim{31.2} & \prelim{56.2} \\
    32 & \prelim{9.4} & \prelim{12.8} & \prelim{22.2} & \prelim{13.2} & \prelim{14.7} & \prelim{27.9} & \prelim{25.1} & \prelim{32.3} & \prelim{57.4} \\
    64 & \prelim{10.7} & \prelim{15.6} & \prelim{26.2} & \prelim{13.1} & \prelim{16.7} & \prelim{29.8} & \prelim{26.5} & \prelim{35.9} & \prelim{62.4} \\
    128 & \prelim{13.8} & \prelim{20.7} & \prelim{34.5} & \prelim{16.1} & \prelim{20.7} & \prelim{36.7} & \prelim{29.1} & \prelim{40.7} & \prelim{69.7} \\
    256 & \prelim{19.9} & \prelim{32.1} & \prelim{52.0} & \prelim{21.8} & \prelim{30.9} & \prelim{52.7} & \prelim{33.6} & \prelim{51.0} & \prelim{84.6} \\
    512 & \prelim{38.7} & \prelim{50.6} & \prelim{89.2} & \prelim{33.6} & \prelim{51.6} & \prelim{85.1} & \prelim{43.9} & \prelim{71.6} & \prelim{115.5} \\
    1024 & \prelim{60.7} & \prelim{89.1} & \prelim{149.8} & \prelim{54.8} & \prelim{90.2} & \prelim{145.0} & \prelim{66.9} & \prelim{111.4} & \prelim{178.3} \\
    2048 & \prelim{105.7} & \prelim{165.2} & \prelim{270.8} & \prelim{96.0} & \prelim{167.2} & \prelim{263.3} & \prelim{117.4} & \prelim{199.1} & \prelim{316.4} \\
    4096 & \prelim{191.5} & \prelim{316.1} & \prelim{507.6} & \prelim{180.1} & \prelim{321.1} & \prelim{501.1} & \prelim{223.9} & \prelim{376.3} & \prelim{600.3} \\


==> generated/table_b300_v41flash.tex <==
    1 & \prelim{8.2} & \prelim{9.1} & \prelim{17.4} & \prelim{14.2} & \prelim{13.3} & \prelim{27.6} & \prelim{23.2} & \prelim{24.7} & \prelim{47.9} \\
    2 & \prelim{9.0} & \prelim{9.5} & \prelim{18.5} & \prelim{13.5} & \prelim{13.2} & \prelim{26.8} & \prelim{21.5} & \prelim{25.6} & \prelim{47.0} \\
    4 & \prelim{8.3} & \prelim{11.6} & \prelim{19.9} & \prelim{13.0} & \prelim{13.3} & \prelim{26.2} & \prelim{21.4} & \prelim{26.1} & \prelim{47.5} \\
    8 & \prelim{8.3} & \prelim{11.7} & \prelim{20.0} & \prelim{14.2} & \prelim{13.6} & \prelim{27.8} & \prelim{21.4} & \prelim{26.5} & \prelim{47.8} \\
    16 & \prelim{8.5} & \prelim{12.1} & \prelim{20.6} & \prelim{13.6} & \prelim{16.0} & \prelim{29.6} & \prelim{21.7} & \prelim{26.8} & \prelim{48.5} \\
    32 & \prelim{9.3} & \prelim{13.5} & \prelim{22.9} & \prelim{13.9} & \prelim{16.8} & \prelim{30.7} & \prelim{22.0} & \prelim{28.2} & \prelim{50.2} \\
    64 & \prelim{10.8} & \prelim{16.3} & \prelim{27.0} & \prelim{14.6} & \prelim{18.2} & \prelim{32.8} & \prelim{23.0} & \prelim{30.6} & \prelim{53.6} \\
    128 & \prelim{13.5} & \prelim{21.7} & \prelim{35.2} & \prelim{17.4} & \prelim{22.2} & \prelim{39.6} & \prelim{25.2} & \prelim{36.5} & \prelim{61.7} \\
    256 & \prelim{20.6} & \prelim{34.5} & \prelim{55.1} & \prelim{23.2} & \prelim{32.5} & \prelim{55.7} & \prelim{30.7} & \prelim{48.0} & \prelim{78.7} \\
    512 & \prelim{37.2} & \prelim{55.7} & \prelim{92.9} & \prelim{35.1} & \prelim{54.1} & \prelim{89.2} & \prelim{42.1} & \prelim{69.3} & \prelim{111.4} \\
    1024 & \prelim{60.4} & \prelim{98.0} & \prelim{158.4} & \prelim{57.4} & \prelim{96.1} & \prelim{153.5} & \prelim{68.9} & \prelim{113.3} & \prelim{182.2} \\
    2048 & \prelim{106.1} & \prelim{180.8} & \prelim{286.9} & \prelim{99.9} & \prelim{178.6} & \prelim{278.5} & \prelim{120.3} & \prelim{205.0} & \prelim{325.3} \\
    4096 & \prelim{197.0} & \prelim{341.7} & \prelim{538.7} & \prelim{188.2} & \prelim{342.4} & \prelim{530.6} & \prelim{227.5} & \prelim{404.1} & \prelim{631.6} \\


==> generated/table_gb200_body.tex <==
    1 & Ours & \textbf{\prelim{35.4}} & \textbf{\prelim{35.4}} & \textbf{\prelim{35.7}} & \textbf{\prelim{36.9}} \\
     & \dedg & \prelim{78.1} & \prelim{78.0} & \prelim{79.1} & \prelim{82.3} \\
     & MegaMoE & \prelim{45.7} & \prelim{46.3} & \prelim{47.2} & \prelim{49.7} \\
    \addlinespace
    16 & Ours & \textbf{\prelim{66.4}} & \textbf{\prelim{51.9}} & \textbf{\prelim{47.7}} & \textbf{\prelim{49.0}} \\
     & \dedg & \prelim{124.5} & \prelim{100.6} & \prelim{88.9} & \prelim{90.9} \\
     & MegaMoE & \prelim{83.4} & \prelim{63.5} & \prelim{58.6} & \prelim{56.0} \\
    \addlinespace
    128 & Ours & \prelim{181.7} & \prelim{124.7} & \prelim{120.9} & \prelim{102.6} \\
     & \dedg & \prelim{237.7} & \prelim{169.3} & \prelim{136.2} & \prelim{126.8} \\
     & MegaMoE & \textbf{\prelim{179.3}} & \textbf{\prelim{121.0}} & \textbf{\prelim{91.2}} & \textbf{\prelim{86.6}} \\


==> generated/table_gb200_layer.tex <==
    8 & 1 & \prelim{35.4} & \prelim{78.1} & \prelim{45.7} & \prelim{40.7} & \prelim{116.5} & \prelim{57.3} \\
     & 16 & \prelim{66.4} & \prelim{124.5} & \prelim{83.4} & \prelim{117.5} & \prelim{200.6} & \prelim{143.8} \\
     & 128 & \prelim{181.7} & \prelim{237.7} & \prelim{179.3} & \prelim{341.5} & \prelim{429.9} & \prelim{344.7} \\
     & 256 & \prelim{208.4} & \prelim{256.9} & \prelim{188.1} & \prelim{491.5} & \prelim{517.4} & \prelim{373.3} \\
     & 512 & \prelim{348.2} & \prelim{317.2} & \prelim{222.0} & \prelim{624.3} & \prelim{728.2} & \prelim{473.1} \\
     & 1024 & \prelim{438.1} & \prelim{481.8} & \prelim{294.1} & \prelim{881.4} & \prelim{1152.7} & \prelim{658.0} \\
     & 4096 & \prelim{1378.8} & \prelim{1457.3} & \prelim{902.4} & \prelim{3123.6}\rlap{$^\dagger$} & \prelim{3537.7} & \prelim{2283.5} \\
    \addlinespace
    16 & 1 & \prelim{35.4} & \prelim{78.0} & \prelim{46.3} & \prelim{43.6} & \prelim{109.5} & \prelim{54.4} \\
     & 16 & \prelim{51.9} & \prelim{100.6} & \prelim{63.5} & \prelim{84.7} & \prelim{151.3} & \prelim{105.4} \\
     & 128 & \prelim{124.7} & \prelim{169.3} & \prelim{121.0} & \prelim{286.0} & \prelim{300.8} & \prelim{214.3} \\
     & 256 & \prelim{200.3} & \prelim{197.2} & \prelim{140.1} & \prelim{395.6} & \prelim{419.1} & \prelim{250.3} \\
     & 512 & \prelim{252.7} & \prelim{272.2} & \prelim{172.1} & \prelim{560.1}\rlap{$^\dagger$} & \prelim{652.5} & \prelim{330.3} \\
     & 1024 & \prelim{440.0} & \prelim{431.4} & \prelim{276.9} & \prelim{1013.3}\rlap{$^\dagger$} & \prelim{1113.8} & \prelim{595.3} \\
     & 4096 & \prelim{1446.6}\rlap{$^\dagger$} & \prelim{1432.2} & \prelim{818.1} & \prelim{3372.0}\rlap{$^\dagger$} & \prelim{3520.2} & \prelim{1885.1} \\
    \addlinespace
    32 & 1 & \prelim{35.7} & \prelim{79.1} & \prelim{47.2} & \prelim{43.7} & \prelim{107.8} & \prelim{53.1} \\
     & 16 & \prelim{47.7} & \prelim{88.9} & \prelim{58.6} & \prelim{66.8} & \prelim{142.9} & \prelim{86.7} \\
     & 128 & \prelim{120.9} & \prelim{136.2} & \prelim{91.2} & \prelim{234.0} & \prelim{258.2} & \prelim{167.0} \\
     & 256 & \prelim{153.0} & \prelim{171.0} & \prelim{114.2} & \prelim{322.0} & \prelim{396.8} & \prelim{207.7} \\
     & 512 & \prelim{265.3} & \prelim{264.8} & \prelim{173.4} & \prelim{570.9}\rlap{$^\dagger$} & \prelim{637.0} & \prelim{340.1} \\
     & 1024 & \prelim{463.8} & \prelim{445.6} & \prelim{265.0} & \prelim{996.3}\rlap{$^\dagger$} & \prelim{1013.9} & \prelim{580.5} \\
     & 4096 & \prelim{1560.7}\rlap{$^\dagger$} & \prelim{1481.1} & \prelim{824.5} & \prelim{3604.2}\rlap{$^\dagger$} & \prelim{3425.8} & \prelim{2018.7} \\
    \addlinespace
    64 & 1 & \prelim{36.9} & \prelim{82.3} & \prelim{49.7} & -- & \prelim{110.3} & \prelim{56.7} \\
     & 16 & \prelim{49.0} & \prelim{90.9} & \prelim{56.0} & -- & \prelim{122.8} & \prelim{74.6} \\
     & 128 & \prelim{102.6} & \prelim{126.8} & \prelim{86.6} & -- & \prelim{242.1} & \prelim{143.2} \\
     & 256 & \prelim{172.8} & \prelim{165.3} & \prelim{112.6} & -- & \prelim{347.6} & \prelim{196.4} \\
     & 512 & \prelim{309.0}\rlap{$^\dagger$} & \prelim{253.3} & \prelim{164.1} & -- & \prelim{567.4} & \prelim{302.3} \\
     & 1024 & \prelim{487.0} & \prelim{422.5} & \prelim{250.9} & -- & \prelim{937.8} & \prelim{524.1} \\
     & 4096 & \prelim{1759.0}\rlap{$^\dagger$} & \prelim{1473.1} & \prelim{789.9} & -- & \prelim{3345.2} & \prelim{1799.4} \\


==> generated/table_gb200_scaling.tex <==
    8 & 1 & \prelim{43.0} & \prelim{17.5} & \prelim{44.7} & \prelim{34.6} & \prelim{17.5} & \prelim{53.6} \\
     & 16 & \prelim{43.1} & \prelim{17.8} & \prelim{44.2} & \prelim{36.0} & \prelim{18.2} & \prelim{57.6} \\
     & 128 & \prelim{48.9} & \prelim{31.7} & \prelim{57.8} & \prelim{44.1} & \prelim{31.5} & \prelim{70.9} \\
     & 1024 & \prelim{160.1} & \prelim{151.6} & \prelim{173.9} & \prelim{150.6} & \prelim{144.0} & \prelim{179.0} \\
    \addlinespace
    16 & 1 & \prelim{41.8} & \prelim{16.6} & \prelim{45.9} & \prelim{48.4} & \prelim{21.5} & \prelim{80.0} \\
     & 16 & \prelim{41.8} & \prelim{18.4} & \prelim{47.1} & \prelim{50.6} & \prelim{23.2} & \prelim{63.5} \\
     & 128 & \prelim{48.8} & \prelim{33.0} & \prelim{61.7} & \prelim{68.1} & \prelim{57.9} & \prelim{92.6} \\
     & 1024 & \prelim{171.5} & \prelim{160.2} & \prelim{186.2} & \prelim{295.0} & \prelim{308.3} & \prelim{335.9} \\
    \addlinespace
    32 & 1 & \prelim{43.2} & \prelim{17.3} & \prelim{48.6} & \prelim{53.7} & \prelim{21.8} & \prelim{73.5} \\
     & 16 & \prelim{44.3} & \prelim{18.2} & \prelim{49.5} & \prelim{57.9} & \prelim{25.4} & \prelim{65.1} \\
     & 128 & \prelim{53.8} & \prelim{34.7} & \prelim{66.4} & \prelim{76.6} & \prelim{61.3} & \prelim{97.1} \\
     & 1024 & \prelim{183.3} & \prelim{169.7} & \prelim{203.1} & \prelim{310.0} & \prelim{320.9} & \prelim{341.6} \\
    \addlinespace
    64 & 1 & \prelim{47.6} & \prelim{17.8} & \prelim{54.2} & \prelim{52.5} & \prelim{23.6} & \prelim{79.1} \\
     & 16 & \prelim{46.7} & \prelim{19.1} & \prelim{55.7} & \prelim{56.0} & \prelim{26.1} & \prelim{90.0} \\
     & 128 & \prelim{58.0} & \prelim{36.7} & \prelim{81.6} & \prelim{78.7} & \prelim{64.2} & \prelim{105.9} \\
     & 1024 & \prelim{191.4} & \prelim{179.8} & \prelim{213.7} & \prelim{320.8} & \prelim{340.6} & \prelim{378.9} \\


==> generated/table_moe_body.tex <==
    \multicolumn{8}{@{}l}{\textit{DeepSeek-V4.1-Flash}} \\
    1 & \prelim{46.0} & \prelim{12.8 / 19.6 / 14.4} & \textbf{\prelim{36.7}} & \prelim{8.3 / 23.9 / 9.8} & \prelim{74.7} & \prelim{21.4 / 26.0 / 27.2} & \prelim{49.8} \\
    16 & \prelim{79.6} & \prelim{13.3 / 49.9 / 17.2} & \textbf{\prelim{70.5}} & \prelim{8.5 / 54.7 / 12.9} & \prelim{122.0} & \prelim{22.0 / 68.7 / 31.4} & \prelim{90.3} \\
    128 & \prelim{188.5} & \prelim{16.3 / 150.0 / 23.1} & \textbf{\prelim{183.3}} & \prelim{13.5 / 150.6 / 21.5} & \prelim{235.9} & \prelim{25.8 / 168.7 / 41.4} & \prelim{188.7} \\
    256 & \prelim{208.1} & \prelim{22.2 / 153.4 / 33.6} & \prelim{206.5} & \prelim{20.5 / 154.9 / 33.8} & \prelim{251.2} & \prelim{29.8 / 170.6 / 50.8} & \textbf{\prelim{194.1}} \\
    1024 & \prelim{353.8} & \prelim{55.2 / 201.3 / 99.2} & \prelim{356.9} & \prelim{60.8 / 206.0 / 96.2} & \prelim{409.6} & \prelim{72.9 / 215.8 / 121.3} & \textbf{\prelim{255.3}} \\
    4096 & \prelim{1185.2} & \prelim{187.2 / 647.9 / 351.6} & \prelim{1198.6} & \prelim{197.4 / 665.7 / 343.3} & \prelim{1290.2} & \prelim{240.1 / 612.1 / 429.6} & \textbf{\prelim{766.1}} \\
    \midrule
    \multicolumn{8}{@{}l}{\textit{Kimi-K3}} \\
    1 & \prelim{47.7} & \prelim{13.1 / 23.5 / 15.1} & \textbf{\prelim{42.1}} & \prelim{8.8 / 28.1 / 13.5} & \prelim{99.7} & \prelim{26.5 / 37.8 / 35.3} & \prelim{60.4} \\
    16 & \prelim{128.4} & \prelim{13.4 / 100.9 / 15.0} & \textbf{\prelim{122.0}} & \prelim{9.4 / 106.5 / 12.5} & \prelim{191.2} & \prelim{23.5 / 129.4 / 38.2} & \prelim{148.6} \\
    128 & \prelim{351.1} & \prelim{17.2 / 313.4 / 21.5} & \textbf{\prelim{346.4}} & \prelim{13.7 / 314.8 / 21.0} & \prelim{430.8} & \prelim{27.0 / 346.9 / 56.8} & \prelim{358.5} \\
    256 & \prelim{396.1} & \prelim{22.8 / 342.2 / 32.0} & \prelim{393.2} & \prelim{20.3 / 343.4 / 32.6} & \prelim{482.1} & \prelim{31.2 / 374.0 / 76.7} & \textbf{\prelim{370.2}} \\
    1024 & \prelim{719.5} & \prelim{54.9 / 561.6 / 102.9} & \prelim{732.1} & \prelim{61.5 / 580.7 / 98.2} & \prelim{976.3} & \prelim{78.1 / 678.5 / 222.3} & \textbf{\prelim{535.8}} \\
    4096 & \prelim{2553.6} & \prelim{181.9 / 2023.0 / 360.2} & \prelim{2601.5} & \prelim{195.8 / 2084.3 / 345.3} & \prelim{3091.1} & \prelim{269.8 / 2006.4 / 817.7} & \textbf{\prelim{1901.9}} \\


==> generated/table_moe_kimik3.tex <==
    1 & \prelim{47.7} & \prelim{13.1 / 23.5 / 15.1} & \prelim{42.1} & \prelim{8.8 / 28.1 / 13.5} & \prelim{60.4} & \prelim{99.7} & \prelim{26.5 / 37.8 / 35.3} \\
    2 & \prelim{52.7} & \prelim{13.0 / 27.8 / 16.0} & \prelim{47.2} & \prelim{8.9 / 32.6 / 14.9} & \prelim{67.5} & \prelim{109.2} & \prelim{26.0 / 45.5 / 37.4} \\
    4 & \prelim{61.8} & \prelim{13.1 / 37.7 / 15.5} & \prelim{57.4} & \prelim{8.9 / 42.6 / 15.2} & \prelim{78.6} & \prelim{120.6} & \prelim{24.2 / 58.3 / 38.2} \\
    8 & \prelim{84.7} & \prelim{14.1 / 59.4 / 15.5} & \prelim{80.7} & \prelim{9.2 / 65.2 / 16.0} & \prelim{106.7} & \prelim{146.2} & \prelim{23.4 / 85.0 / 37.8} \\
    16 & \prelim{128.4} & \prelim{13.4 / 100.9 / 15.0} & \prelim{122.0} & \prelim{9.4 / 106.5 / 12.5} & \prelim{148.6} & \prelim{191.2} & \prelim{23.5 / 129.4 / 38.2} \\
    32 & \prelim{211.9} & \prelim{13.5 / 183.5 / 15.9} & \prelim{206.4} & \prelim{9.7 / 189.4 / 13.9} & \prelim{231.2} & \prelim{281.8} & \prelim{24.4 / 216.4 / 41.0} \\
    64 & \prelim{334.5} & \prelim{14.8 / 303.2 / 17.6} & \prelim{328.9} & \prelim{10.7 / 309.4 / 16.3} & \prelim{350.9} & \prelim{416.0} & \prelim{25.5 / 344.2 / 46.3} \\
    128 & \prelim{351.1} & \prelim{17.2 / 313.4 / 21.5} & \prelim{346.4} & \prelim{13.7 / 314.8 / 21.0} & \prelim{358.5} & \prelim{430.8} & \prelim{27.0 / 346.9 / 56.8} \\
    256 & \prelim{396.1} & \prelim{22.8 / 342.2 / 32.0} & \prelim{393.2} & \prelim{20.3 / 343.4 / 32.6} & \prelim{370.2} & \prelim{482.1} & \prelim{31.2 / 374.0 / 76.7} \\
    512 & \prelim{515.6} & \prelim{33.8 / 419.3 / 58.8} & \prelim{515.3} & \prelim{38.9 / 423.8 / 54.1} & \prelim{418.4} & \prelim{620.6} & \prelim{46.2 / 451.5 / 121.5} \\
    1024 & \prelim{719.5} & \prelim{54.9 / 561.6 / 102.9} & \prelim{732.1} & \prelim{61.5 / 580.7 / 98.2} & \prelim{535.8} & \prelim{976.3} & \prelim{78.1 / 678.5 / 222.3} \\
    2048 & \prelim{1342.9} & \prelim{97.7 / 1060.3 / 189.7} & \prelim{1367.5} & \prelim{109.6 / 1093.9 / 179.3} & \prelim{1007.5} & \prelim{1789.6} & \prelim{138.8 / 1232.6 / 422.6} \\
    4096 & \prelim{2553.6} & \prelim{181.9 / 2023.0 / 360.2} & \prelim{2601.5} & \prelim{195.8 / 2084.3 / 345.3} & \prelim{1901.9} & \prelim{3091.1} & \prelim{269.8 / 2006.4 / 817.7} \\


==> generated/table_moe_v41flash.tex <==
    1 & \prelim{46.0} & \prelim{12.8 / 19.6 / 14.4} & \prelim{36.7} & \prelim{8.3 / 23.9 / 9.8} & \prelim{49.8} & \prelim{74.7} & \prelim{21.4 / 26.0 / 27.2} \\
    2 & \prelim{47.9} & \prelim{12.8 / 21.2 / 14.6} & \prelim{39.2} & \prelim{8.9 / 26.6 / 9.8} & \prelim{52.4} & \prelim{80.5} & \prelim{21.8 / 28.4 / 30.0} \\
    4 & \prelim{51.2} & \prelim{12.3 / 25.5 / 14.2} & \prelim{44.6} & \prelim{8.1 / 29.7 / 12.1} & \prelim{57.8} & \prelim{85.8} & \prelim{21.6 / 34.4 / 29.8} \\
    8 & \prelim{59.5} & \prelim{13.1 / 32.4 / 14.7} & \prelim{52.1} & \prelim{8.5 / 37.2 / 11.9} & \prelim{68.1} & \prelim{98.4} & \prelim{21.9 / 46.1 / 30.4} \\
    16 & \prelim{79.6} & \prelim{13.3 / 49.9 / 17.2} & \prelim{70.5} & \prelim{8.5 / 54.7 / 12.9} & \prelim{90.3} & \prelim{122.0} & \prelim{22.0 / 68.7 / 31.4} \\
    32 & \prelim{113.3} & \prelim{13.5 / 83.2 / 17.8} & \prelim{105.8} & \prelim{9.1 / 88.7 / 14.2} & \prelim{123.0} & \prelim{160.2} & \prelim{22.7 / 104.4 / 33.2} \\
    64 & \prelim{177.9} & \prelim{13.5 / 146.6 / 18.9} & \prelim{171.8} & \prelim{10.4 / 147.1 / 16.2} & \prelim{184.7} & \prelim{227.4} & \prelim{23.6 / 168.1 / 35.7} \\
    128 & \prelim{188.5} & \prelim{16.3 / 150.0 / 23.1} & \prelim{183.3} & \prelim{13.5 / 150.6 / 21.5} & \prelim{188.7} & \prelim{235.9} & \prelim{25.8 / 168.7 / 41.4} \\
    256 & \prelim{208.1} & \prelim{22.2 / 153.4 / 33.6} & \prelim{206.5} & \prelim{20.5 / 154.9 / 33.8} & \prelim{194.1} & \prelim{251.2} & \prelim{29.8 / 170.6 / 50.8} \\
    512 & \prelim{259.3} & \prelim{33.2 / 170.5 / 57.0} & \prelim{260.5} & \prelim{37.5 / 171.5 / 53.9} & \prelim{214.9} & \prelim{300.3} & \prelim{44.7 / 181.0 / 74.4} \\
    1024 & \prelim{353.8} & \prelim{55.2 / 201.3 / 99.2} & \prelim{356.9} & \prelim{60.8 / 206.0 / 96.2} & \prelim{255.3} & \prelim{409.6} & \prelim{72.9 / 215.8 / 121.3} \\
    2048 & \prelim{637.9} & \prelim{99.6 / 355.5 / 184.5} & \prelim{645.1} & \prelim{106.2 / 363.3 / 179.8} & \prelim{428.3} & \prelim{672.3} & \prelim{127.8 / 320.2 / 224.3} \\
    4096 & \prelim{1185.2} & \prelim{187.2 / 647.9 / 351.6} & \prelim{1198.6} & \prelim{197.4 / 665.7 / 343.3} & \prelim{766.1} & \prelim{1290.2} & \prelim{240.1 / 612.1 / 429.6} \\


==> generated/table_precision.tex <==
    \multicolumn{7}{@{}l}{\textit{DeepSeek-V4.1-Flash}} \\
    BF16 & BF16 & 10288\,/\,10240 & 29.0 & 46.3 & 194.3 & 684.5 \\
    MXFP8 & BF16 & 5328\,/\,10240 & 28.7 & 40.7 & 154.9 & 532.7 \\
    FP8 (1$\times$128) & BF16 & 5328\,/\,10240 & 28.6 & 41.1 & 155.3 & 532.7 \\
    NVFP4 & BF16 & 2928\,/\,10240 & 28.1 & 37.6 & 137.4 & 456.0 \\
    MXFP8 & FP8 & 5328\,/\,5120 & 28.0 & 39.9 & 131.4 & 438.9 \\
    \midrule
    \multicolumn{2}{@{}l}{MXFP8, at the source} & 5328\,/\,10240 & 30.4 & 43.4 & 158.9 & 547.7 \\
    \multicolumn{2}{@{}l}{BF16, at the target} & 10288\,/\,10240 & 30.6 & 48.8 & 214.2 & 768.1 \\
    \midrule
    \multicolumn{7}{@{}l}{\textit{Kimi-K3}} \\
    BF16 & BF16 & 7296\,/\,7168 & 25.6 & 42.7 & 183.5 & 644.0 \\
    MXFP8 & BF16 & 3824\,/\,7168 & 25.0 & 37.7 & 146.5 & 502.0 \\
    FP8 (1$\times$128) & BF16 & 3824\,/\,7168 & 25.1 & 37.6 & 146.6 & 502.2 \\
    NVFP4 & BF16 & 2144\,/\,7168 & 24.8 & 35.2 & 128.8 & 430.1 \\
    MXFP8 & FP8 & 3824\,/\,3584 & 24.3 & 36.5 & 124.2 & 419.9 \\
    \midrule
    \multicolumn{2}{@{}l}{MXFP8, at the source} & 3824\,/\,7168 & 26.4 & 40.3 & 149.7 & 514.5 \\
    \multicolumn{2}{@{}l}{BF16, at the target} & 7296\,/\,7168 & 25.2 & 42.7 & 196.8 & 701.8 \\


==> generated/table_skew_body.tex <==
    1 & 0 & \prelim{1.50} & \prelim{16.1} & \prelim{47.6} & \prelim{52.2} & \prelim{97.5} & \prelim{68.3} & \prelim{1.38} & \prelim{22.4} & \prelim{58.0} & \prelim{84.6} & \prelim{148.0} & \prelim{114.2} \\
     & 0.5 & \prelim{1.50} & \prelim{15.8} & \prelim{49.4} & \prelim{57.8} & \prelim{105.2} & \prelim{73.0} & \prelim{1.25} & \prelim{28.2} & \prelim{68.5} & \prelim{81.0} & \prelim{146.1} & \prelim{106.8} \\
     & 1 & \prelim{1.50} & \prelim{15.8} & \prelim{52.6} & \prelim{52.4} & \prelim{99.3} & \prelim{67.6} & \prelim{1.38} & \prelim{30.0} & \prelim{65.4} & \prelim{71.1} & \prelim{133.4} & \prelim{96.6} \\
     & 1.25 & \prelim{1.67} & \prelim{15.9} & \prelim{51.6} & \prelim{52.3} & \prelim{97.9} & \prelim{69.2} & \prelim{1.62} & \prelim{22.1} & \prelim{62.2} & \prelim{66.4} & \prelim{129.4} & \prelim{95.4} \\
    \addlinespace
    1024 & 0 & \prelim{1.02} & \prelim{119.5} & \prelim{178.4} & \prelim{414.9} & \prelim{461.1} & \prelim{255.6} & \prelim{1.01} & \prelim{143.0} & \prelim{291.7} & \prelim{717.6} & \prelim{968.6} & \prelim{538.9} \\
     & 0.5 & \prelim{1.29} & \prelim{125.7} & \prelim{199.8} & \prelim{445.4} & \prelim{499.5} & \prelim{303.9} & \prelim{1.19} & \prelim{131.3} & \prelim{306.7} & \prelim{852.3} & \prelim{1096.7} & \prelim{638.9} \\
     & 1 & \prelim{1.69} & \prelim{146.4} & \prelim{242.3} & \prelim{557.0} & \prelim{626.7} & \prelim{374.4} & \prelim{1.55} & \prelim{134.2} & \prelim{373.0} & \prelim{1075.3} & \prelim{1352.6} & \prelim{814.0} \\
     & 1.25 & \prelim{1.91} & \prelim{160.4} & \prelim{267.1} & \prelim{619.4} & \prelim{696.0} & \prelim{411.5} & \prelim{1.70} & \prelim{134.7} & \prelim{400.0} & \prelim{1184.5} & \prelim{1477.0} & \prelim{918.4} \\


==> generated/table_zipf.tex <==
    Perfect & 1 & \prelim{36.7} & \prelim{74.7} & \prelim{49.8} & \prelim{0.74} & \prelim{1.00} & \prelim{42.1} & \prelim{99.7} & \prelim{60.4} & \prelim{0.70} & \prelim{1.00} \\
     & 16 & \prelim{70.5} & \prelim{122.0} & \prelim{90.3} & \prelim{0.78} & \prelim{1.00} & \prelim{122.0} & \prelim{191.2} & \prelim{148.6} & \prelim{0.82} & \prelim{1.00} \\
     & 128 & \prelim{183.3} & \prelim{235.9} & \prelim{188.7} & \prelim{0.97} & \prelim{1.00} & \prelim{346.4} & \prelim{430.8} & \prelim{358.5} & \prelim{0.97} & \prelim{1.00} \\
     & 1024 & \prelim{353.8}\rlap{$^\dagger$} & \prelim{409.6} & \prelim{255.3} & \prelim{1.39} & \prelim{1.00} & \prelim{719.5}\rlap{$^\dagger$} & \prelim{976.3} & \prelim{535.8} & \prelim{1.34} & \prelim{1.00} \\
    \addlinespace
    Zipf, $\alpha=0$ & 1 & \prelim{52.2} & \prelim{97.5} & \prelim{68.3} & \prelim{0.76} & \prelim{1.50} & \prelim{84.6} & \prelim{148.0} & \prelim{114.2} & \prelim{0.74} & \prelim{1.38} \\
     & 16 & \prelim{154.1} & \prelim{208.8} & \prelim{167.3} & \prelim{0.92} & \prelim{1.09} & \prelim{302.9} & \prelim{387.8} & \prelim{328.7} & \prelim{0.92} & \prelim{1.23} \\
     & 128 & \prelim{188.8}\rlap{$^\dagger$} & \prelim{233.7} & \prelim{188.8} & \prelim{1.00} & \prelim{1.03} & \prelim{347.5} & \prelim{432.3} & \prelim{359.0} & \prelim{0.97} & \prelim{1.03} \\
     & 1024 & \prelim{414.9} & \prelim{461.1} & \prelim{255.6} & \prelim{1.62} & \prelim{1.02} & \prelim{717.6}\rlap{$^\dagger$} & \prelim{968.6} & \prelim{538.9} & \prelim{1.33} & \prelim{1.01} \\
    \addlinespace
    Zipf, $\alpha=0.5$ & 1 & \prelim{57.8} & \prelim{105.2} & \prelim{73.0} & \prelim{0.79} & \prelim{1.50} & \prelim{81.0} & \prelim{146.1} & \prelim{106.8} & \prelim{0.76} & \prelim{1.25} \\
     & 16 & \prelim{154.6} & \prelim{209.0} & \prelim{165.1} & \prelim{0.94} & \prelim{1.31} & \prelim{295.5} & \prelim{376.3} & \prelim{320.2} & \prelim{0.92} & \prelim{1.36} \\
     & 128 & \prelim{204.2} & \prelim{250.2} & \prelim{196.1} & \prelim{1.04} & \prelim{1.25} & \prelim{386.7} & \prelim{456.4} & \prelim{384.9} & \prelim{1.00} & \prelim{1.20} \\
     & 1024 & \prelim{445.4}\rlap{$^\dagger$} & \prelim{499.5} & \prelim{303.9} & \prelim{1.47} & \prelim{1.29} & \prelim{852.3}\rlap{$^\dagger$} & \prelim{1096.7} & \prelim{638.9} & \prelim{1.33} & \prelim{1.19} \\
    \addlinespace
    Zipf, $\alpha=1$ & 1 & \prelim{52.4} & \prelim{99.3} & \prelim{67.6} & \prelim{0.77} & \prelim{1.50} & \prelim{71.1} & \prelim{133.4} & \prelim{96.6} & \prelim{0.74} & \prelim{1.38} \\
     & 16 & \prelim{142.2} & \prelim{179.5} & \prelim{140.5} & \prelim{1.01} & \prelim{1.62} & \prelim{257.5} & \prelim{322.8} & \prelim{273.7} & \prelim{0.94} & \prelim{1.59} \\
     & 128 & \prelim{233.8} & \prelim{279.2} & \prelim{221.1} & \prelim{1.06} & \prelim{1.67} & \prelim{445.8} & \prelim{539.1} & \prelim{449.1} & \prelim{0.99} & \prelim{1.56} \\
     & 1024 & \prelim{557.0} & \prelim{626.7} & \prelim{374.4} & \prelim{1.49} & \prelim{1.69} & \prelim{1075.3}\rlap{$^\dagger$} & \prelim{1352.6} & \prelim{814.0} & \prelim{1.32} & \prelim{1.55} \\
    \addlinespace
    Zipf, $\alpha=1.25$ & 1 & \prelim{52.3} & \prelim{97.9} & \prelim{69.2} & \prelim{0.76} & \prelim{1.67} & \prelim{66.4} & \prelim{129.4} & \prelim{95.4} & \prelim{0.70} & \prelim{1.62} \\
     & 16 & \prelim{132.1} & \prelim{163.2} & \prelim{129.7} & \prelim{1.02} & \prelim{1.93} & \prelim{218.0} & \prelim{274.0} & \prelim{233.9} & \prelim{0.93} & \prelim{1.70} \\
     & 128 & \prelim{240.0} & \prelim{289.7} & \prelim{225.8} & \prelim{1.06} & \prelim{1.91} & \prelim{447.1} & \prelim{550.0} & \prelim{453.5} & \prelim{0.99} & \prelim{1.71} \\
     & 1024 & \prelim{619.4} & \prelim{696.0} & \prelim{411.5} & \prelim{1.51} & \prelim{1.91} & \prelim{1184.5}\rlap{$^\dagger$} & \prelim{1477.0} & \prelim{918.4} & \prelim{1.29} & \prelim{1.70} \\

